Fusing information streams in end-to-end audio-visual speech recognition

End-to-end acoustic speech recognition has quickly gained widespread popularity and shows promising results in many studies. Specifically the joint transformer/CTC model provides very good performance in many tasks. However, under noisy and distorted conditions, the performance still degrades notably. While audio-visual speech recognition can significantly improve the recognition rate of end-to-end models in such poor conditions, it is not obvious how to best utilize any available information on acoustic and visual signal quality and reliability in these models. We thus consider the question of how to optimally inform the transformer/CTC model of any time-variant reliability of the acoustic and visual information streams. We propose a new fusion strategy, incorporating reliability information in a decision fusion net that considers the temporal effects of the attention mechanism. This approach yields significant improvements compared to a state-of-the-art baseline model on the Lip Reading Sentences 2 and 3 (LRS2 and LRS3) corpus. On average, the new system achieves a relative word error rate reduction of 43% compared to the audio-only setup and 31% compared to the audiovisual end-to-end baseline.

==> Section/delete.tex <==
Different from \cite{afouras2018deep}, which combine the context vectors, in our project the additional reliability indicators are extracted and used to get a better models fusion performance. 

Often, stream weighting proved to be an effective method to combine audio and video information in hybrid model. As in \cite{meutzner2017improving}, separate models are then trained for each of the modalities, and possibly, for each of the feature streams per modality. Stream weighting is realized through a weighted combination of the DNN state posteriors of each modality
\begin{equation} \label{statefusion}
\textnormal{log }\widetilde{p}(s |\textbf{o}_t)=\sum_{i}^{}\lambda_t^i\cdot \textrm{log }{p}(s |\textbf{o}_t^{i}),
\end{equation}
where $\textrm{log }{p}(s |\textbf{\textrm{o}}_t^{i})$ is the log-posterior of state $s$ in stream $i$ and $\textnormal{log}\,\widetilde{p}(s |\textbf{\textrm{o}}_t)$ is its estimated combined log-posterior.
The stream weights $\lambda_t^i$ are typically predicted by appropriate reliability measures. In this paper, we propose a new way to use stream weighting on TM-CTC based AVSR model.



The probabilities are fused via

\begin{equation} \label{TMstatefusion}
\textnormal{log }\widetilde{p}_{s2s}(s |\textbf{o}_m)=\lambda^{a}_{m}\cdot \textrm{log }{p_{s2s}}(s |\textbf{o}_m^{a}) + \lambda^{v}_{m}\cdot \textrm{log }{p_{s2s}}(s |\textbf{o}_m^{v})
\end{equation}
and
\begin{equation} \label{CTCstatefusion}
\textnormal{log }\widetilde{p}_{ctc}(s |\textbf{o}_n)=\gamma^{a}_{n}\cdot \textrm{log }{p_{ctc}}(s |\textbf{o}_n^{a}) + \gamma^{v}_{n}\cdot \textrm{log }{p_{ctc}}(s |\textbf{o}_n^{v}).
\end{equation}



Then we use a weightnet predict the weights for each model. The weightnet has 2 hidden layers, with 128, 64 units, respectively. Each using ReLU activation functions, the output is the predicted weight for each stream $\lambda^{i}_{m}$. A sigmoid function is used to limite the weights to value between 0 and 1. 
\begin{equation} \label{tmpred}
\lambda^{i} = \textrm{sigmoid}(\textrm{weightnet}(R_i)).
\end{equation}
Finally, we normalize the fused multi-modal S2S probabilities to one for each character. 

The CTC weights estimation is much easier, since the $rms^{i}_{out}$ and $P_{ctc}$ have the same length.
\begin{equation} \label{ctcpred}
\gamma^{i} = \textrm{sigmoid}(\textrm{weightnet}(rms^{i}_{out})).
\end{equation}




\begin{equation} \label{atrans1}
\textbf{T}_a = \textrm{softmax}(\frac{(\textbf{W}_a^Q\textbf{Q}_a^T)\cdot (\textbf{W}_a^K\textbf{K}_a^{T})^T}{\sqrt{d_k}}),
\end{equation}

\begin{equation} \label{atrans2}
\textbf{T}_v = \textrm{softmax}(\frac{(\textbf{W}_v^Q\textbf{Q}_v^T)\cdot (\textbf{W}_v^K\textbf{K}_v^{T})^T}{\sqrt{d_k}}),
\end{equation}
where $\textbf{Q}_a$ and $\textbf{K}_a$ are the queries and keys from the audio attention block and $\textbf{Q}_v$ and $\textbf{K}_v$ are from video attention block.



As shown in Tab. \ref{table:rms}, 

\begin{table}[]
    \caption{Proposed reliability measures}
\label{table:rms}
    %\small    
    \footnotesize
    %\scriptsize
% shorten the intercolumn spaces
    \setlength\tabcolsep{2.0pt}
    \centering
\begin{tabular}{|c|c|}
\hline
Audio-based                                                                                                        & Video-based \\ \hline
\begin{tabular}[c]{@{}l@{}}\tabitem MFCCs\\ \tabitem SNR\\ \tabitem Pitch\\ \tabitem $\Delta $ pitch\\ \tabitem Probability of voicing\end{tabular} &  \begin{tabular}[c]{@{}l@{}} \tabitem Confidence  \\ \tabitem AUs \end{tabular} \\ \hline
\end{tabular}
\end{table}  

\subsection{Audio-based reliability measures}
The low order MFCC coefficients are related to the audio quality. It has also reported that MFCC coefficients are help for voice activity detection \cite{kinnunen2007voice}. Here the first 7 MFCC coefficients are used.


 The audio-visual model baseline (in Sec. \ref{avbaseline}) was trained for 100 epochs and took around 9 days.
 
 
\iffalse
\subsection{Dataset}

\begin{table}[]
    \caption{Dataset}
\label{table:dataset}
    %\small    
    \footnotesize
    %\scriptsize
% shorten the intercolumn spaces
    \setlength\tabcolsep{2.0pt}
    \centering
\begin{tabular}{|c|c|c|}
\hline
                  & Utt.    & Vocab. \\ \hline
LRS2-pretrain set & 96,318  & 41,427 \\ 
LRS2-training set & 45,839  & 17,660 \\ 
LRS2-test set     & 1,243   & 1,698  \\ \hline
LRS3-pretrain set & 118,516 & 51k    \\ \hline
\end{tabular}
\end{table}

Our experiments are based on the LRS2 \cite{afouras2018deep} and LRS3 corpus \cite{afouras2018lrs3}. As we know that lip-reading task is harder than audio speech recognition. Therefore, the LRS2 and LRS3 pretrain sets are use for AVSR system pretraining. Then the model is fine tuning on LRS2 training set and test on test set. The statistics of these sets are given in Tab. \ref{table:dataset}.

\subsection{Data augmentation} \label{dataaug}
Data augmentation can be divided into two parts, audio and visual visual data augmentation, respectively. As mentioned before, audio speech recognition is easier than lip-reading task, in AVSR system, the recognition performance is usually dominate by acoustic model. Hence, to avoid this problem and analyze the performance in different acoustic noise environments, we artificially apply the audio data augmentation to the raw audio signal. The MUSAN corpus \cite{snyder2015musan} is used as noise dataset. The ambient and music noise are used with seven different SNR, from -9 dB to 9 dB in steps of 3 dB. Each audio signal is augmented with these two noise types and the SNR is randomly chosen from all SNR. In addition, we also create reverb noise for some audio signals. 

The similar visual data augmentation in \cite{stafylakis2017combining} is also performed in visual sequences, i.e. random cropping and horizontal flips with probability 50\%.

\subsection{Feature extraction}
The audio model uses 80 log Mel features together with pitch, delta pitch and probability of voicing as features (all 83 features), audio features are extracted with 25 ms frame size and 10 ms frame shift. The video feature is the mouth image, it is 96 $\times$ 96 pixel grayscale mouth region of interest (ROI) and detected via OpenFace \cite{baltruvsaitis2016openface}. The video frame is 40 ms long without overlap.


\subsection{Pretrained model}
The video and AVSR model are pretrained on LRS2 and LRS3 pretrain sets. Nevertheless, training model with a such large dataset is unpractical. Therefore, during pretrain stage, the visual feature extractor parameters are frozen. Then fine tune all the parameters in model with LRS2 training set. 

\subsection{Language model}
The language model is trained by a 4 unidirectional layers recurrent network, each layer contains 2048 units. In this project we use the language model, which is trained on Librispeech corpus \cite{panayotov2015librispeech}. The language model predicts one character each time and receives the previous character as the input. 

\subsection{DGX}

\fi


In addition, we also create reverb noise for some audio signals by convolutions with measured impose responses. These impulse responses also come from the MUSAN corpus.


\begin{table}[!htbp]
\centering
        \footnotesize

 \caption{WER: Fine-tuning on LRS2 training set. \textbf{AO}: audio-only model. \textbf{VO}: video-only model.\textbf{AV}: baseline model \cite{afouras2018deep}. \textbf{DFN}: our proposed model. \textbf{m}: music noise. \textbf{a}:ambient oise. \textbf{gb}: visual augmentation Gaussian blur. \textbf{sp}: visual augmentation salt-and-pepper noise. \\textbf{vc}: clean visual data}
 \setlength\tabcolsep{1.0pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular*}{\linewidth}{cccccccccccc|c}

&-12 &-9 &-6 &-3 &0 &3 &6 &9 &12 &clean &reverb &avg. \\
AO(m) &21.0 &21.3 &14.0 &13.3 &15.0 &11.3 &8.2 &7.0 &6.6 &8.8 &10.5 &12.45\\
AO(a) &29.8 &25.6 &23.0 &14.5 &12.8 &10.8 &9.0 &9.2 &8.7 &8.8 &10.5 &14.79\\
VO(vc) &58.7 &61.0 &61.7 &69.6 &69.6 &63.5 &64.6 &63.6 &66.6 &61.9 &61.9 &63.88\\
VO(gb) &66.6 &69.2 &71.0 &68.5 &68.5  &71.1 &62.7 &69.4 &67.6 &66.9 &66.9 &68.04\\
VO(sp) &68.5 &72.5 &73.7 &70.1 &70.1  &70.6 &68.3 &69.1 &73.1 &67.9 &67.9 &70.16\\
\midrule
AV(m.vc) &14.6 &11.8 &6.4 &7.9 &7.9 &6.3 &5.2 &4.4 &3.4 &4.0 &5.8 &7.06\\
AV(a.vc) &19.1 &19.0 &14.3 &7.3 &6.3 &6.0 &5.7 &4.5 &4.9 &4.0 &5.8 &8.81\\
AV(a.gb) &20.6 &18.9 &15.0 &7.7 &6.8 &7.5 &5.9 &3.9 &4.8 &4.0 &6.0 &9.19\\
AV(a.sp) &19.5 &19.9 &15.3 &7.7 &7.2 &6.3 &5.6 &4.4 &4.6 &4.3 &6.0 &9.16\\
\midrule
DFN(m.vc) &11.1 &8.7 &5.5 &4.8 &4.8 &4.5 &3.6 &3.3 &2.2 &2.4 &3.6 &\textbf{4.95}\\
DFN(a.vc) &14.3 &11.9 &8.1 &4.8 &4.0 &5.4 &3.7 &2.8 &3.6 &2.4 &3.6 &\textbf{5.87}\\
DFN(a.gb) &14.9 &12.8 &9.4 &5.2 &4.2 &5.5 &3.8 &3.0 &4.1 &2.6 &3.8 &\textbf{6.29}\\
DFN(a.sp) &15.4 &12.8 &9.9 &5.2 &4.7 &5.5 &3.4 &2.6 &4.0 &2.5 &3.7 &\textbf{6.34}\\

%\hline 
\end{tabular*}
\label{table:espnetresults}
\end{table}


As described in Sec. \ref{decoder}, $\textbf{Q}$ comes from the $\textbf{C}$ with size nToken $\times$ 256, where nToken is the length of the transcription. $\textbf{K}$ and $\textbf{V}$ are from $\textbf{Enc}_{out}^i$ and have a size $(\textrm{nFrames}/4)\times 256$ (since the subsampling layer and Bresnham's algorithm). In Eq. \ref{dotatt}, $\textbf{T}_j$ converts $\textbf{V}$ from size $(\textrm{nFrames}/4)\times 256$ to nToken $\times$ 256. The attention transform matrix $\textbf{T}_j$ shows  how important the current features for the current transcription. 

In Fig. \ref{fig:decoders}, in the transformer decoder, there are 6 multi-head attention blocks, each of them has an attention transform matrix, we use the transform matrix from the last block to convert $\textbf{rms}_{out}$ from size $(\textrm{nFrames}/4)\times 256$ to nToken $\times$ 256. Because in the last block, $\textbf{Q}$ attends better to $\textbf{K}$. In each head, the audio reliability indicators  ($\textbf{rms}^{a}_{out}$) and the video reliability indicators ($\textbf{rms}^{v}_{out}$) are converted via
\begin{equation} \label{convert}
\textbf{R}_j^a = \textbf{T}_j^a \cdot (\textbf{W}_j^{arms}\textbf{rms}^{a}_{out})^T,\textbf{R}_j^v = \textbf{T}_j^v \cdot (\textbf{W}_j^{vrms}\textbf{rms}^{v}_{out}).
\end{equation}
$\textbf{R}^i$ is the concatenated output of each head ($\textbf{R}_j^i$) and projected by a feed-forward layer. 

==> Section/dnn.tex <==
\begin{tikzpicture}
    \node (naveq) [naveqs] {DFN};
    % Note the use of \path instead of \node at ... below. 
    \path (naveq.65)+(-\blockdistdnn,0) node (input1) {${p}(\textbf{s} |\textbf{o}^a)$};
    \path (naveq.35)+(-\blockdistdnn,0) node (input2) {${p}(\textbf{s} |\textbf{o}^v)$};
    \path (naveq.-65)+(-\blockdistdnn,0) node (input3) {$\textbf{R}^v$ or $\textbf{rms}_{out}^v$};
    \path (naveq.-35)+(-\blockdistdnn,0) node (input4) {$\textbf{R}^a$ or $\textbf{rms}_{out}^a$};
    
    
    \path [draw, ->] (input1) -- node [above] {} 
        (naveq.west |- input1) ;
    \path [draw, ->] (input2) -- node [above] {} 
        (naveq.west |- input2) ;
    \path [draw, ->] (input3) -- node [above] {} 
        (naveq.west |- input3) ;
    \path [draw, ->] (input4) -- node [above] {} 
        (naveq.west |- input4) ;
        
    \path (naveq.0)+(\edgedistdnn,0) node (input5) {$\textnormal{log }p(\textbf{s} |\textbf{o})$};
    \path [draw, <-] (input5) -- node [above] {} 
        (naveq.east |- input5) ;        
 
\end{tikzpicture}




==> Section/framework.tex <==
\begin{tikzpicture}[scale=0.7,transform shape]
  % Draw diagram elements
 
  \path \result {1}{$\textnormal{log }\widetilde{p}(\textbf{s} |\textbf{o}_t)$};
  \path (p1.south)+(0.0,-1.0) \practica{111}{Log-Softmax};
  \path (p111.south)+(0.0,-1.0) \practica{2}{FC};
  \path (p2.south)+(0.0, -1.0) \practica{3}{Tanh Dropout};
  \path (p3.south)+(0.0,-1.0) \practica{4}{3 BLSTMs};
    \path (p4.south)+(0.0, -1.0) \practica{8}{LN ReLU Dropout};
  \path (p8.south)+(0.0,-1.0) \practica{9}{Hidden Layer};

  \path (p9.south)+(0.0,-1.0) \resultlarge{10}{${p}(\textbf{s} |\textbf{o}_t^{\mathrm{A}}),{p}(\textbf{s} |\textbf{o}_t^{\mathrm{VA}}),{p}(\textbf{s} |\textbf{o}_t^{\mathrm{VS}}), \textbf{R}_t$};

  
  
  \draw [<-] (p1.south) -- node [above] {} (p111);
  \draw [<-] (p111.south) -- node [above] {} (p2);
  %\draw [<-] (p2.west) -- +(-1.0em, 0) |- node [above] {} (p3.east) ;
  \draw [<-] (p2.south) -- node [above] {} (p3);
  \draw [<-] (p3.south) -- node [above] {} (p4);
  \draw [<-] (p8.south) -- node [above] {} (p9);                    
  \draw [<-] (p9.south) -- node [above] {} (p10);                    
  %\draw [<-] (p4.west) -- +(-1.0em, 0) |- node [above] {} (p8.east) ;
  \draw [<-] (p4.south) -- node [above] {} (p8);                    
\begin{pgfonlayer}{background} 
 \node[draw, thick, dotted, fill=yellow!50, rounded corners, draw=black!50, dashed, inner xsep=0.3em, inner ysep=0.3em, fit=(p8) (p9)] (armbox) {};
 \node at (armbox.north east)[right]{$\times$ 3};
 %\node[draw, thick, dotted, rounded corners, inner xsep=1.9em, inner ysep=0.6em, fit=(p111)(p9)] (abox) {};
 %\node at (abox.north east)[right]{Fusion Net};
\end{pgfonlayer}
% \path[fill=yellow!20,rounded corners, draw=black!50, dashed] (a) rectangle (b);

  
\end{tikzpicture}




==> Section/removed.tex <==
The audio and video model are trained separately. 

Before introducing the new fusion strategy, the size of some variables should be declared. In Fig. \ref{fig:encoders}, assuming the $\textbf{o}^a$ is $\textrm{nFrames}$ length, the $\textbf{Enc}_{out}^a$, $\textbf{Enc}_{out}^v$ and $\textbf{rms}_{out}$ have the same size $(\textrm{nFrames}/4)\times 256$ (since subsampling layer and Bresenham's algorithm). So, in Fig. \ref{fig:decoders}, the size of $\textbf{Enc}_{out}^i$ is $(\textrm{nFrames}/4)\times 256$. For transformer decoder, the $\textbf{C}$ has size nToken $\times$ 256, where nToken is the length of the transcription. (nFrames/4) is not euqal to nToken. Finally, \textbf{C} is projected by a fully connected layer, so the $p_{s2s}(\textbf{s} |\textbf{o})$ has size nToken $\times$ $d_{out}$, where $d_{out}$ is the output dimension, it is depended on the dictionary. Comparing the $\textbf{rms}_{out}$ and $p_{s2s}(\textbf{s} |\textbf{o})$, they have different length. In transformer decoder, the feature length changes because of the attention mechanisms.


In Fig. \ref{fig:Feedforward}, $F_1=2048$ and $F_2$=256.

==> diagram/feedforward.tex <==
\begin{tikzpicture}[scale=0.6,transform shape]
  \path \resultindex {1}{$\textbf{Out}$};
  \path (p1.south)+(0.0,-1.0) \practica{2}{Layer Normalization};
  \path (p2.south)+(0.0,-1.0) \add{3}{+};
  \path (p3.south)+(0.0,-1.0) \practica{4}{Linear Layer $F_2$ + ReLU};
  \path (p4.south)+(0.0,-1.0) \practica{5}{Linear Layer $F_1$ + ReLU};
  \path (p5.south)+(0.0,-1.0) \resultindex{7}{$\textbf{X}$};
  
  
  \draw [-{Latex[length=1mm, width=2mm]}] (p2.north) -- node [above] {} (p1);
 \draw [-{Latex[length=1mm, width=2mm]}] (p3.north) -- node [above] {} (p2);  
 \draw [-{Latex[length=1mm, width=2mm]}] (p4.north) -- node [above] {} (p3);
 \draw [-{Latex[length=1mm, width=2mm]}] (p5.north) -- node [above] {} (p4); 
 \draw [-{Latex[length=1mm, width=2mm]}] (p7.north) -- node [above] {} (p5); 
 %\draw [-{Latex[length=1mm, width=2mm]}] (p7.north) -- node [above] {} (p6);
 
\draw[-{Latex[length=1mm, width=2mm]}] (p7.west) -- +(-4.0em, 0) |- (p3.west);
 

 \path (p1.west)+(-6.0,0.0) \resultindex{11}{$\textbf{X}$};
  \path (p11.south)+(0.0,-1.0) \practica{12}{Layer Normalization};
  \path (p12.south)+(0.0,-1.0) \add{13}{+};
  \path (p13.south)+(0.0,-1.0) \practica{14}{Multi-head Attention};
  \path (p14.south)+(0.0,-1.0) \resultindex{15}{$\textbf{K}$};
  \path (p14.south)+(-1.3,-1.0) \resultindex{16}{$\textbf{V}$};
  \path (p14.south)+(1.3,-1.0) \resultindex{17}{$\textbf{Q}$};
  %\path (p14.south)+(3.0,-1.0) \result{18}{$Residual$};
  \draw [-{Latex[length=1mm, width=2mm]}] (p12.north) -- node [above] {} (p11);  
   \draw [-{Latex[length=1mm, width=2mm]}] (p13.north) -- node [above] {} (p12);   
  \draw [-{Latex[length=1mm, width=2mm]}] (p14.north) -- node [above] {} (p13);  
   \draw [-{Latex[length=1mm, width=2mm]}] (p15.north) -- node [above] {} (p14);
     \draw [-{Latex[length=1mm, width=2mm]}] (p16.north) -- node [above] {} (p14);  
   \draw [-{Latex[length=1mm, width=2mm]}] (p17.north) -- node [above] {} (p14);  
  \draw[-{Latex[length=1mm, width=2mm]}] (p17.east) -- +(0.5em, 0) |- (p13.east);  
  \node[draw, thick, dotted, rounded corners, inner xsep=1.2em, inner ysep=0.3em, fit=(p12) (p14)] (attbox) {};  
 \node[draw, thick, dotted, rounded corners, inner xsep=1.2em, inner ysep=0.3em, fit=(p2) (p5)] (armbox) {};


\end{tikzpicture}


